Uniqueness of Equilibria in Interactive Networks

This paper extends the unified network model, proposed by Acemoglu et al. (2016b), such that interaction functions can be heterogeneous, and the sensitivity matrix has less than or equal to one spectral radius. We show the existence and (almost surely) uniqueness of equilibrium under both eventually contracting and noncontracting assumptions. Applying the equilibrium in the study of systemic risk, we provide a measure to determine the key player who causes the most significant impact if removed from the network.

==> algorithm2.tex <==
\begin{algorithm}[!htb]
% \DontPrintSemicolon
\SetAlgoNoEnd%
\SetAlFnt{\tiny}
\SetAlCapNameFnt{\small}
\SetAlCapFnt{\small}
\SetKwProg{try}{try}{}{}
\SetKwProg{except}{except}{}{}
\caption{Compute equilibrium given the interaction functions (\ref{eq:bounded identity map}).}\label{algorithm_2}
% \KwIn{$f, W, \e, u, \ell, n, N$}
% \KwOut{$x^{(t)}$: equilibrium }
$t\gets 0$;  $x^{(-1)} \gets u$; $A_{-1} \gets \{1, \dots, n \}$; $A_{0} \gets A(u)$\;
\While{$A_t \neq A_{t-1}$}
{   
$t\gets t + 1$\;
    \try{}{
    $x^{(t)} \gets \max\{ 
    [u \Lambda^{A_t} + (u\Lambda^{A_t} W  + \e) (I - \Lambda^{A_t})][I - (I-\Lambda^{A_t}) W(I - \Lambda^{A_t})]^{-1}, \ell\}
    $\;
    }
    \lexcept{}{\textbf{break}}
    $A_{t} \gets A(x^{(t)})$\;
}
\If{$x^{(t)} \neq f(x^{(t)}W + \e)$}{
    $A_0 \gets \{i\in N: x^{(t)}_i \geq u_i \}$\;
    $x^a \gets x^{(t)}$;
    $x^{-1} \gets \ell$;
    $B_{-1} \gets \{1, \dots, n\}$;
    $B_{0} \gets B(\ell)$\;
    
    \While{$E_t \neq E_{t-1}$}{
    $t\gets t + 1$\;
    \try{}{
    $x^{(t)} \gets \min\{[\ell \Lambda^{B_t} + (\ell\Lambda^{B_t} W+ \e)(I - \Lambda^{B_t})][I - (I - \Lambda^{B_t}) W (I - \Lambda^{B_t})]^{-1}, u\}$
    }
    \lexcept{}{ \textbf{break}}
     $B_{t} \gets B(x^{(t)})$\;
    }
 \If{$x^{(t)} \neq f(x^{(t)} W + \e)$}{
    $B_0 \gets \{i \in N \colon x^{(t)}_i \leq \ell_i \}$\;
    \lIf{$|B_0|\leq |A_0| $}{$\mathcal{P} \gets \text{ the power set of } B_0$} 
    \lElse{$\mathcal{P} \gets \text{ the power set of } A_0$}
    
\For{$i=0;\ i < |\mathcal{P}|; \ i=i+1$}{
\If{$|B_0|\leq |A_0| $}{
$\hat{u} \gets \ell \Lambda^{P_i} + u (I - \Lambda^{P_i}) , \text{ where } P_i \subset  B_0 \text{ is the $i$-th element of } \mathcal{P}$\;
$A_t \gets A(\hat{u}) \cap (N\setminus P_i)$; 
$B_t \gets P_i$\;
}
\Else{
$\hat{\ell} \gets \ell (I - \Lambda^{P_i}) + u \Lambda^{P_i} , \text{ where } P_i \subset  A_0 \text{ is the $i$-th element of } \mathcal{P}$\;
$B_t \gets B(\hat{\ell}) \cap (N\setminus P_i)$; 
$A_t \gets P_i$\;
}

\For{$j=0; \ j < n; \ j = j+1$}{
    $t \gets t+1$\;
    % $x^{(t)} \gets None$\;
    \try{}{
    $x^{(t)} \gets \text{ the fixed point of }$ $x = u \Lambda^{A_{t-1}} + \ell \Lambda^{B_{t-1}} + [u \Lambda^{A_{t-1}} W + \ell \Lambda^{B_{t-1}} W +  x (I -\Lambda^{A_{t-1}} -  \Lambda^{B_{t-1}}) W + \e](I -\Lambda^{A_{t-1}} -  \Lambda^{B_{t-1}}) $\;
    }
    \lexcept{}{
   \textbf{break}
    }
    
    \lIf{$|B_0|\leq |A_0| $}{$A_t \gets A(x^{(t)})$; $B_t \gets B_{0}$}
    \lElse{$B_t \gets B(x^{(t)})$; $A_t \gets A_{0}$}
    
    \lIf{$A_t = A_{t-1}$ \textbf{and} $B_t = B_{t-1}$ }{
    \textbf{break}}
    }
\lIf{$x^{(t)} = f(x^{(t)} W + \e)$}{\Return $x^{(t)}$}    
    }   
}
}
\end{algorithm}
